Motion Planning on Visual Manifolds

In this thesis, we propose an alternative characterization of the notion of Configuration Space, which we call Visual Configuration Space (VCS). This new characterization allows an embodied agent (e.g., a robot) to discover its own body structure and plan obstacle-free motions in its peripersonal space using a set of its own images in random poses. Here, we do not assume any knowledge of geometry of the agent, obstacles or the environment. We demonstrate the usefulness of VCS in (a) building and working with geometry-free models for robot motion planning, (b) explaining how a human baby might learn to reach objects in its peripersonal space through motor babbling, and (c) automatically generating natural looking head motion animations for digital avatars in virtual environments. This work is based on the formalism of manifolds and manifold learning using the agent's images and hence we call it Motion Planning on Visual Manifolds.

==> abstract.tex <==

Humans and most other animals are very good at avoiding obstacles and navigating in complex environments just by visually observing the world. They routinely use the prior sensorimotor experience to build motor models and use vision for gross motor tasks in novel environments. Achieving similar abilities in robots, without having to calibrate a robot’s own body structure, or estimate exact 3-D positions, is a touchstone problem 
for robotics.

The notion of Configuration Space (also known as C-Space) is fundamental to conceptualizing multibody motion and to address the problem of Robot Motion Planning -- planning obstacle-free paths from a source configuration to a destination configuration. Traditional solutions to the motion planning problem involve constructing an explicit representation of the robot in terms of the number of degrees of freedom, joint and link geometry, rules for forward kinematics and inverse kinematics to map from the configuration space to the work-space and vice versa. Once such a representation is available, obstacle-free paths can be planned in the configuration space. This approach is quite cumbersome because different representations need to be hand-engineered for different robots, obstacles, and workspaces. If we consider the triple (robot, obstacles, workspace) as a system, the traditional approach is quite system specific. Any change in the system would require operating on a different hand-engineered model.

In this thesis, we propose an alternative characterization of configuration space, which we call the Visual Configuration Space (VCS), to address the motion planning problem. Beginning with a dense enough set of images of the robot in random configurations, it is possible to discover the topology of its motion manifold, using manifold learning methods such as Isomap. This is possible because, in spite of the robot images being very high-dimensional, the governing parameters of its motion are much fewer and as a result, the robot images can only change in very restricted ways. This manifold, discovered using the robot images, is the visual configuration space.  A path between two configurations of the robot is a curve between the corresponding points on the VCS. Since we can only use a finite sample of images, we will only have a discrete representation of the VCS, which we call the Visual Roadmap (VRM). The VRM is a graph in which each node corresponds to an image of the robot in some configuration with an edge between two nodes whose poses are near-by according to some metric in the image space. We use the VRM to compute shortest paths between configurations. We discuss the conditions under which the visual configuration space is homeomorphic to the canonical C-Space. We also discuss how obstacles in the workspace are mapped on to VCS and VRM and the issues involved in 
and the advantages of using the VRM for motion planning.

We apply the framework of VCS in three different contexts: (i) robot motion planning, where we present empirical results related to robot motion planning for various types of simulated planar robots and some real 3-D robots; (ii) modeling body schema for infant motor learning, where we discuss how a cognitive agent acquires a representation of its body that allows it to infer the position and orientation of its limbs relative to its world, and to move and perform actions in that world; and (iii) generating head motion animations for avatars in virtual environments.
